A Framework for Differential Privacy Against Timing Attacks

The standard definition of differential privacy (DP) ensures that a mechanism's output distribution on adjacent datasets is indistinguishable. However, real-world implementations of DP can, and often do, reveal information through their runtime distributions, making them susceptible to timing attacks. In this work, we establish a general framework for ensuring differential privacy in the presence of timing side channels. We define a new notion of timing privacy, which captures programs that remain differentially private to an adversary that observes the program's runtime in addition to the output. Our framework enables chaining together component programs that are timing-stable followed by a random delay to obtain DP programs that achieve timing privacy. Importantly, our definitions allow for measuring timing privacy and output privacy using different privacy measures. We illustrate how to instantiate our framework by giving programs for standard DP computations in the RAM and Word RAM models of computation. Furthermore, we show how our framework can be realized in code through a natural extension of the OpenDP Programming Framework.

==> postprocessing.tex <==
\section{Post-Processing of Timing-Private Programs}
A fundamental property of differential privacy is that it is preserved under post-processing (Lemma ~\ref{lem:dp postprocess}). Arbitrary transformations applied to differentially private outputs produces new outputs that remain differentially private. Unfortunately, the definition of timing privacy is incompatible with post processing. Timing privacy bounds the \emph{additional} information leakage caused by observing the program's running time after observing the program's output. However, post processing can potentially destroy information in the program's output and this can result in unbounded additional information leakage in the program's runtime.

To see this effect in action, consider a jointly output/timing-pure program $P$ implementing the identity function $f(x) = x$ with the additional property that the runtime reveals something about the input. That is, $\TP{x} = g(x)$ for a non-constant function $g$. Then $P$ is $(1\mapsto 0)$-timing-private with respect to the change-one distance metric $d_{CO}$ and any privacy measure $\mathcal{M}$ (e.g., max divergence). The identity function program satisfies perfect timing privacy despite its running time being directly correlated with its input. This is due to the fact that $P$'s output already reveals the input and so the program's running time reveals no additional information. However, if we apply the simple post-processing step $f'$ that sets $f'(\out(P(x, \env)), \TP{x, \env}) = (0, \TP{x, \env})$, then the result is no longer perfectly timing-private since $\TP{x, \env}$ leaks information about the input (everything about it if $g$ is injective). 
